Metareasoning for Planning Under Uncertainty

The conventional model for online planning under uncertainty assumes that an agent can stop and plan without incurring costs for the time spent planning. However, planning time is not free in most real-world settings. For example, an autonomous drone is subject to nature's forces, like gravity, even while it thinks, and must either pay a price for counteracting these forces to stay in place, or grapple with the state change caused by acquiescing to them. Policy optimization in these settings requires metareasoning---a process that trades off the cost of planning and the potential policy improvement that can be achieved. We formalize and analyze the metareasoning problem for Markov Decision Processes (MDPs). Our work subsumes previously studied special cases of metareasoning and shows that in the general case, metareasoning is at most polynomially harder than solving MDPs with any given algorithm that disregards the cost of thinking. For reasons we discuss, optimal general metareasoning turns out to be impractical, motivating approximations. We present approximate metareasoning procedures which rely on special properties of the BRTDP planning algorithm and explore the effectiveness of our methods on a variety of problems.

==> extramath.tex <==
We must compute $E[Q(s, a_j) | \rightarrow a_j] = $
\begin{align*}
& \int P(Q^b(s, a_i) | \rightarrow a_j) Q^b(s, a_i) dQ^b(s, a_i)\\
=& \int \frac{P(\rightarrow a_j | Q^b(s, a_i) )P(Q^b(s, a_i))}{P(\rightarrow a_j)} Q^b(s, a_i) dQ^b(s, a_i)\\
=& \frac{1}{P(\rightarrow a_j)}\int P(\rightarrow a_j | Q^b(s, a_i) )P(Q^b(s, a_i))Q^b(s, a_i) dQ^b(s, a_i)\\
\end{align*}

In the case where $Q$ is given by upper bounds and $a_i \neq a_j$, we have
\begin{align*}
E[Q^b(s, a_i) | \rightarrow a_j] &= \frac{P(Q^b(s, a_i))}{P(\rightarrow a_j)}\int P(\rightarrow a_j | Q^b(s, a_i) )Q^b(s, a_i) dQ^b(s, a_i)\\
\end{align*}
There are three cases. If $Q^b(s, a_i) >= u_{a_j}$, 
\begin{align*}
P(\rightarrow a_j | Q^b(s, a_i) ) &= 1\\
\end{align*}
If $l_{a_j} <= Q^b(s, a_i) < u_{a_j}$:
\begin{align*}
P(\rightarrow a_j | Q^b(s, a_i) ) &= \frac{Q^b(s, a_i) - l_{a_j}}{u_{a_j} - l_{a_j}}\\
\end{align*}
And if $Q^b(s, a_i) < l_{a_j}$:
\begin{align*}
P(\rightarrow a_j | Q^b(s, a_i) ) &= 0
\end{align*}
Therefore, we have
\begin{align*}
E[Q^b(s, a_i) | \rightarrow a_j] &= \frac{P(Q^b(s, a_i))}{P(\rightarrow a_j)}[\int_{Q^b(s, a_i) >= u_{a_j}} Q^b(s, a_i) dQ^b(s, a_i)\\
&+ \int_{l_{a_j} <= Q^b(s, a_i) < u_{a_j}} \frac{Q^b(s, a_i) - l_{a_j}}{u_{a_j} - l_{a_j}} Q^b(s, a_i) dQ^b(s, a_i) ]\\
&= \frac{P(Q^b(s, a_i)}{P(\rightarrow a_j)}[\frac{1}{2}Q^b(s, a_i)^2 \biggr\arrowvert_{Q^b(s, a_i) >= u_{a_j}} \\
&+ \frac{1}{u_{a_j} - l_{a_j}} [\frac{1}{3}Q^b(s, a_i)^3 - \frac{l_{a_j}}{2}Q^b(s, a_i)^2 ]\biggr\arrowvert_{l_{a_j} <= Q^b(s, a_i) < u_{a_j}}]\\
\end{align*}


In the case when $a_i == a_j$, we have
\begin{align*}
E[Q^b(s, a_j) | \rightarrow a_j] &= \frac{P(Q^b(s, a_j))}{P(\rightarrow a_j)}[\int_{Q^b(s, a_j) >= u_{a_j}} Q^b(s, a_j) dQ^b(s, a_j)\\
&+ \int_{l_{a_j} <= Q^b(s, a_i) < u_{a_j}} \frac{Q^b(s, a_i) - l_{a_j}}{u_{a_j} - l_{a_j}} Q^b(s, a_i) dQ^b(s, a_i) ]\\
\end{align*}
There are again three cases. If $Q^b(s, a_j) >= u_{a_i}$, 
\begin{align*}
P(\rightarrow a_j | Q^b(s, a_j) ) &= 0\\
\end{align*}
If $l_{a_i} <= Q^b(s, a_j) < u_{a_i}$:
\begin{align*}
P(\rightarrow a_j | Q^b(s, a_j) ) &= \frac{u_{a_i} - Q^b(s, a_j)}{u_{a_i} - l_{a_i}}\\
\end{align*}
And if $Q^b(s, a_j) < l_{a_i}$:
\begin{align*}
P(\rightarrow a_j | Q^b(s, a_j) ) &= 1
\end{align*}
Therefore, we have
\begin{align*}
E[Q^b(s, a_j) | \rightarrow a_j] &= \frac{P(Q^b(s, a_j))}{P(\rightarrow a_j)}[\int_{Q^b(s, a_j) \leq l_{a_i}} Q^b(s, a_j) dQ^b(s, a_j)\\
&+ \int_{l_{a_i} \leq Q^b(s, a_j) < u_{a_i}} \frac{u_{a_i} - Q^b(s, a_j)}{u_{a_i} - l_{a_i}} Q^b(s, a_j) dQ^b(s, a_j) ]\\
&= \frac{P(Q^b(s, a_j)}{P(\rightarrow a_j)}[\frac{1}{2}Q^b(s, a_j)^2 \biggr\arrowvert_{Q^b(s, a_j) \leq l_{a_i}} \\
&+ \frac{1}{u_{a_i} - l_{a_i}} [\frac{u_{a_i}}{2}Q^b(s, a_j)^2 - \frac{1}{3}Q^b(s, a_j)^3]\biggr\arrowvert_{l_{a_i} \leq Q^b(s, a_j) < u_{a_i}}]\\
\end{align*}


We can then integrate by parts by letting $u = P(\rightarrow a_j | Q^b(s, a_i) )$ and $dv = P(Q^b(s, a_i))Q^b(s, a_i)$.
\begin{align*}
E[Q^b(s, a_i) | \rightarrow a_j] &= \frac{1}{P(\rightarrow a_j)} [P(\rightarrow a_j | Q^b(s, a_i) ) E[Q^b(s, a_i)]\biggr\arrowvert_{l_{a_i}}^{u_{a_i}} - E[Q^b(s, a_i)]\int  \frac{dP(\rightarrow a_j | Q^b(s, a_i) )}{dQ^b(s, a_i)} dQ^b(s, a_i)] \\
&= \frac{E[Q^b(s, a_i)]}{P(\rightarrow a_j)} [P(\rightarrow a_j | Q^b(s, a_i) )  \biggr\arrowvert_{l_{a_i}}^{u_{a_i}} - [u(u_{a_i}) - u(l_{a_i})]]
\end{align*}
We have
\begin{eqnarray*}
\frac{dP(\rightarrow a_j | Q^b(s, a_i) )}{dQ^b(s, a_i)} &=& \frac{d (1-g_j(Q^bs, a_i))}{dQ^b(s, a_i)}\\
&-& 
\end{eqnarray*}


\subsection{Correlated Bounds}



\begin{align*}
P(\rightarrow a_j) &=& \int_{l_{a_i}}^{u_{a_i}} P(Q^b(s,a_i))  \prod_j P(Q^b(s, a_j) > P(Q^b(s, a_i)) dQ^b(s, a_i)\\
&=& \int_{l_{a_i}}^{u_{a_i}} f_i(Q^b(s, a_i))\prod_j (1-g_j(Q^b(s, a_j)))dQ^b(s, a_i)
\end{align*}
where $f_i(x)$ and $g_j(x)$ are the pdf and cdf of the Irwin-Hall distributions, respectively.
When the number of cycles $y=1$, the computation reduces to  
\begin{align*}
P(\rightarrow a_j) &=& \frac{1}{u_{a_i} - u_{a_j}}\int_{l_{a_i}}^{u_{a_i}} \prod_j \frac{u_{a_j} - Q^b(s, a_i)}{u_{a_j} - l_{a_j}} dQ^b(s, a_i),
\end{align*} which has a closed form solution.

\subsection{Approaches that attempt to estimate the improvement in policy from planning and compare it against the cost of planning}
\begin{itemize}
\item Try to exploit simple regret bounds provided by some algorithms (e.g., BRUE). If the improvement in policy is greater than the cost of planning, then plan. 
\begin{algorithm}
\caption{Myopic Regret MetaPlan}
\label{algorithm}
\begin{algorithmic}
\Require $Y$ the number of computational cycles each action provides, Planner $P: \mathbb{Z} \rightarrow \mathbb{R}$ that takes the number of total number of planning cycles and outputs an upper-bound on regret, total cycles of planning so-far, $y$, current policy, $\pi_y$, current state $s$
\State
\State Compute the 1-step change in regret $\Delta R =  P(y) - P(y + Y(\texttt{NOP}))$
\If {$\Delta R > C(\texttt{s, NOP})$}
\State \Return \texttt{NOP}
\Else
\State \Return $\pi_y(s)$.
\EndIf 
\end{algorithmic}
\end{algorithm}
\item Use upper and lower bounds for the value function (easily obtainable). Assume if thinking, the best improvement will occur. If this best improvement is greater than the cost of thinking, then think.



\begin{algorithm}
\caption{Optimistic Non-Myopic Planning MetaPlan - computes an upper bound on the improvement of V(S)}
\label{algorithm}
\begin{algorithmic}
%\Require Planner $P: \mathbb{Z} \rightarrow Q^{\pi_y}_U \times Q^{\pi_y}_L$ that takes the number of total number of planning cycles and outputs upper and lower bounds on the Q-function, total cycles of planning so-far, $y$, current policy, $\pi_y$, current state $s$
%\State
\State Compute $\Delta = \min_{a} Q^{\pi_y}_U(s, a) - \min_{a} Q^{\pi_y}_L(s, a) $
\If {$\Delta > C(\texttt{s, NOP})$}
\State \Return \texttt{NOP}
\Else
\State \Return $\pi_y(s)$.
\EndIf 
\end{algorithmic}
\end{algorithm}

\begin{itemize}
\item The difference between second policy and the first policy is that the the first policy is eager, and the second conservative. The first is myopic, and the second not.

\item We can estimate policy improvement curves by doing more planning. (exploration vs exploitation tradeoff)
\end{itemize}



==> oldstuff.tex <==
\comment{
\section{Estimating VOC for BRTDP}

Per discussion in Section \ref{sec:theory}, $B$ may explore its configuration space in any order, and provide no indication of the quality of the policies it considers.  Since approximating $Q^*(s^m, f(s,\chi))$ and $Q^*(s^m, \texttt{NOP})$ requires assessing policy values, we seek an algorithm that efficiently provides the value of policies with some guarantees. We find that Bounded RTDP (BRTDP) \cite{mcmahan-icml05} has such desirable properties.

BRTDP is an anytime planning algorithm based on RTDP \cite{barto-aij95}. BRTDP provides upper and lower bounds on the optimal value function, $V^*$, and updates these bounds as it runs. The initial bounds are rooted in two heuristics. Just like RTDP, BRTDP chooses actions greedily w.r.t. the lower (admissible) bound when running trials, providing guarantees about convergence to the optimal policy. In contrast to RTDP, if BRTDP is stopped in advance of converging, it returns an action greedy w.r.t. the upper bound.  Desirable properties of BRTDP's are captured in the following theorem \Bug{Andrey to self:Verify the source!}:

\begin{theorem}\cite{mcmahan-icml05}\label{thm:brtdp} If BRTDP  is initialized with a \emph{monotone} upper-bound heuristic, the expected cost of the policy greedy w.r.t. the upper bound at any time until BRTDP converges is no worse than the upper bound. A monotone upper bound monotonically decreases as BRTDP runs. A monotone lower bounds monotonically increases as BRTDP runs.
\end{theorem}

The monotone value function of an MDP decreases under Bellman backup updates if it is an upper bound on $V^*$ and increases if it is a lower bound. While Theorem \ref{thm:brtdp} does \emph{not} imply that the expected cost of the policy greedy w.r.t. to a monotone upper bound monotonically drops as BRTDP progresses, the upper-bound value function provides information on how poor the policy could be. The construction of domain-independent monotone bounds is beyond the scope of this paper; we shall describe the design of monotone or near-monotone bounds for the domains in our empirical evaluation. Moving ahead, we assume that BRTDP bounds are monotone.

\comment{
BRTDP must be given initial upper and lower bounds on the optimal value function. An upper bound is \emph{monotone} if after every Bellman backup, the upper bound decreases. Although constructing a monotone upper bound heuristic is not always trivial, our algorithms assume that the upper bounds are monotone. In many domains, including the ones we experiment on, monotone upper bounds are trivially constructed. Similarly, a lower bound is monotone if after every Bellman backup, the lower bound increases.
}


Because BRTDP selects actions using its maintained upper bounds on the value function, we compute the expected upper bound (UB) on the value of computation rather than the expected value of computation:

\begin{align*}
E^{UB}[VOC(s^m)] =& E^{UB}[Q(s^m, f(s,\chi)) - Q(s^m, \texttt{NOP})]  \\
\end{align*}

\subsection{Estimating Terms using Upper Bounds}
We now show how we can compute terms efficiently by making assumptions about BRTDP.
\subsubsection{Estimating $P(\rightarrow a_j)$ }

Let $\hat{\Delta}_{s,a}$  be the change in the upper and lower bounds of action $a$ in state $s$ in the most recent planning cycle. As a first assumption, we assert that the change resulting from an additional cycle of planning, $\Delta_{s,a}$, will be no larger than the last change, $\Delta_{s,a} \leq \hat{\Delta}_{s,a}$.

To represent our uncertainty in the next change, we assume a distribution $D$ over changes such that $\Delta_{t} \sim D[0, \Delta_{t+1}]$. A candidate informationless prior is the uniform distribution. With this assumption, computing $P(\rightarrow a_j)$ consists of computing an integral of a polynomial of degree $|A|$, and thus computing $P(\rightarrow a_j)$ for all actions $j$ can be computed in time $O(|A|^2)$.  

A weakness of this approach is that changes in the upper-bounds for different actions are modeled independently, when they are dependent in practice. For example, if the upper bounds for two actions decrease by a large amount in the previous time step, then it is unlikely that in the next timestep, one upper bound will drop dramatically while the other drops very little at all. Thus, the amount of uncertainty in the upper-bound at the next time-step is overestimated, and the value of computation will be overestimated. Thus, we would like to jointly model the changes in upper-bounds for all actions.  With this end in mind, we assume that all ratios between future drops in the next thinking cycle are equal to the ratios between the observed drops in the last thinking cycle. Formally, we draw $\rho \sim$ Uniform[0, 1]. Then, let $\Delta_{s,a} = \rho \cdot \hat{\Delta}_{s,a}$ for all states $s$ and actions $a$. Given these assumptions, we can view each action $a_j$ as a line segment on the unit interval [0,1] where $a_j(0) = u_{s,a}$ and $a_j(1) = u_{s,a} - \Delta_{s,a_j}$. $P(\rightarrow a_j)$ is simply the proportion of the line representing $a_j$ which lies underneath all other lines. One can naively compute these probabilities in time $O(|A|^2)$ by enumerating all intersections. 

We speed up computations by considering only a constant number of actions.  Thus, the computation is gated by the time the algorithm takes to select these actions to compare. We choose the two actions with the lowest potential upper bounds, leading to a linear algorithm with time complexity linear in the number of actions, $O(|A|)$.   


%will result in a change of $\Delta_{t+1} \sim Uniform[0, \Delta_t]$. We use a uniform distribution to represent no knowledge about how the bound may change, and we assume that the change $\Delta_{t+1}$  cannot be greater than the last change.

%where $f_i(x)$ and $g_j(x)$ are the pdf and cdf of the distributions, respectively. 
%\begin{eqnarray*}
%P(\rightarrow a_j) &=& \frac{1}{u_{a_i} - u_{a_j}}\int_{l_{a_i}}^{u_{a_i}} \prod_j \frac{u_{a_j} - Q^b(s, a_i)}{u_{a_j} - l_{a_j}} dQ^b(s, a_i),
%\end{eqnarray*} which has a closed form solution.

\subsubsection{Estimating $E[Q(s^m, a_j)]$}
When estimate Q-values in a greedy manner; at each metarasoning step, we assume that the agent does not perform any more computation in the future. Formally, instead of estimating $E[Q(s^m, a_j)]$, we estimate $E[Q^M(s, a_j)]$.
With this additional assumption, approximating $E[Q(s, a_j)]$ is simple. The Q-value is simply the mean of the line segment representing action $a_j$:
\begin{align*}
E[Q(s, a_j)] = a_j(0) - \frac{|a_j(0) - a_j(1)|}{2}.
\end{align*}

\subsubsection{Estimating $E[Q(s^m, a_j) | \rightarrow a_j]$}
Finally, we show how to compute $E[Q(s^m, a_j) | \rightarrow a_j]$. We again perform a greedy computation. When we assume the actions are uncorrelated, we have $E[Q(s, a_j) | \rightarrow a_j] = $
\begin{align*}
\int{Q(s,a_j) \frac{P(\rightarrow a_j | Q(s, a_j)) P(Q(s, a_j))}{P(\rightarrow a_j)} dQ(s, a_i)}.
\end{align*}
Since we fix the number of actions we consider to 2, computation of this integral takes constant time. Given that the planner switches to action $a_j$, the expected Q-value is the mean of the portion of the line segment representing $a_j$ that is beneath all other lines. Letting $0 \leq  x < y \leq 1$ represent the endpoints of the segment with minimum Q-value, we have:
\begin{align*}
E[Q(s, a_j)] = a_j(x) - \frac{|a_j(x) - a_j(y)|}{2}.
\end{align*}

\subsection{Putting it all Together}
The pseudocode of the metareasoning algorithm is presented in Algorithm \ref{algorithm}.  The core of the algorithm involves the computations we describe in the previous section. In experiments, we denote \texttt{UnCorr Metareasoner} as the metareasoner that assumes the actions are uncorrelated, and \texttt{Metareasoner} as the metareasoner that does not. Both algorithms take time linear in the number of actions. To complete the algorithm, we add a few key details. We note that our algorithm decides to plan for another cycle if $\hat{\Delta}_{s,a}$ does not yet exist, as metareasoning about actions for which you have no information about is unreasonable. 


\begin{algorithm}
\caption{General Metareasoner}
\label{algorithm}
\begin{algorithmic}
\State Compute $\hat{u}_{s,a} = u_{s,a} - \hat{\Delta}_{s,a}$ for all actions $a$
\State Let $\hat{A}$ be the set of 2 actions with the lowest $\hat{u}$.
\If {$\hat{\Delta}_{s,a}$ does not exist for any action $a \in \hat{A}$}
\State \Return \texttt{NOP}
\EndIf
\State Approximate $\hat{V} = E^{UB}[VOC(s, \sigma)] $
\If {$\hat{V} > 0$}
\State \Return \texttt{NOP}
\Else
\State \Return \texttt{EXECUTE}.
\EndIf 
\end{algorithmic}
\end{algorithm}
}



Then, the agent can compute its expected value of computation:
\begin{align*}
E[VOC(s^m)] =& E[Q(s^m, f(s,\chi)) - Q(s^m, \texttt{NOP})].  \\
\end{align*}
Now, let $\rightarrow a_j$ denote the event that the new policy after a cycle of thinking in configuration state $\sigma$ will recommend action $a_j$ in state $s$. %Formally, $P(\rightarrow a_j) = \sum_{\sigma'}\tau(\sigma, \sigma')\mathbbm{1}_{\pi^{\sigma'}}(a_j)$. 
and let $\chi'$ be the random variable denoting the configuration state that is transitioned to. Then, by taking the \emph{single-step} assumption \cite{russell-aij91} that taking a \texttt{NOP} represents a \emph{complete computation}, a computation that results in a commitment to a base action, 
$E[Q(s^m, \texttt{NOP})]$ =
\begin{align*}
&= \sum_{s'} T(s, \texttt{NOP}, s') \sum_{j} P(\rightarrow a_j)  E[Q((s, \chi'), a_j) | \rightarrow a_j].\\
\end{align*}

In either case, our goal then, is to compute or approximate the quantities $P(\rightarrow a_j)$, $E[Q(s^m, a_j)]$, and $E[ Q(s^m, a_j) | \rightarrow a_j]$. These quantities $P(\rightarrow a_j) =$
\begin{align*}
\int P(Q(s^m,a_j))  \prod_i P(Q(s^m, a_i) > P(Q(s^m, a_j)) dQ(s^m, a_j),\\
%&=& \int_{l_{a_i}}^{u_{a_i}} f_i(Q^b(s, a_i))\prod_j (1-g_j(Q^b(s, a_j)))dQ^b(s, a_i)
\end{align*}
$E[Q(s^m, a_j) = $
\begin{align*}
\int P(Q(s^m, a_i)) Q(s^m, a_i) dQ(s^m, a_i)\\
\end{align*}
and $E[Q(s^m, a_j) | \rightarrow a_j] = $
\begin{align*}
\int P(Q(s^m, a_i) | \rightarrow a_j) Q(s^m, a_i) dQ(s^m, a_i)\\
\end{align*}
in general cannot be naively computed efficiently.
 
We do not propose an algorithm to compute these quantities efficiently in the general case. Instead, we consider the case of a particular planning algorithm, and make a number of modeling assumptions for this algorithm in order to make metareasoning tractable. We now review the planner that we use in our case study, Bounded Real-Time Dynamic Programming (BRTDP). 

\comment{
This is where BRTDP's properties help us again. To start with, let us assume that one ``thinking cycle'' of BRTDP (i.e., executing \texttt{NOP} once and running BRTDP in the meantime) corresponds to completing some fixed number of BRTDP trials from the agent's current world state $s$ so that each of these trials starts with the \texttt{NOP} action. Running these trials updates the values of $\overline{V}$ and $\underline{V}$ for some states, and hence $\overline{Q}$ and $\underline{Q}$ for some state-action pairs. Note, in fact, that \emph{BRTDP's new configuration $\chi'$ after a thinking cycle is uniquely determined by the agent's world state $s'$ after executing \texttt{NOP} and the updated $\overline{Q}$ and $\underline{Q}$ for all state-action pairs.} Denote the Q-value bounds corresponding to BRTDP's new configuration $\chi'$ as $\overline{Q}^{\chi'}$.

\begin{align}\label{eq:approxQafut}
Q^{\chi'}(s', a) \approx E[\mathcal{Q}^{\chi'}(s', a)].
\end{align}

\noindent
The reason we derived the estimates of $Q^{\chi'}(s', a)$ is that knowing $Q^{\chi'}(s', a)$ for all actions in $s'$ finally lets us compute $V^{\chi'}(s')$, needed for Equation \ref{eq:qnopapprox}:

\begin{align}\label{eq:maxact}
V^{\chi'}(s') = \max_a Q^{\chi'}(s', a).
\end{align}

To recap the logic behind our approximation scheme so far, \emph{if} an agent in world state $s$ knew in advance the new bounds $\overline{Q}^{\chi'}$ that running BRTDP for one thinking cycle would yield, it could evaluate $Q^*(s^m, \texttt{NOP})$ by making a few approximations and plugging an estimate for $V^{\chi'}(s')$ (Equation \ref{eq:maxact}) into Equation \ref{eq:qnopapprox}. Coupled with an estimate for $Q^*(s^m, f(s,\chi))$ obtained earlier (Equation \ref{eq:approxQa}), this would allow the agent to make an informed metareasoning decision via Equations \ref{eq:voc} and \ref{eq:obs}. 

The trouble, however, is that the bounds $\overline{Q}^{\chi'}$ and aren't known beforehand. They depend on BRTDP's configuration-to-configuration transition function $T^{B(M)}(\chi, \chi')$, which is random (although, as mentioned in Section 3, it can be de-randomized by simulating BRTDP on a deterministic Turing machine). Put differently, $\overline{Q}^{\chi'}$  is actually sampled from random variables $\overline{\mathcal{Q}}^{\chi'}$ whose distributions are unknown. Fortunately, we can estimate them for any action $a$ in the state $s'$ where \texttt{NOP} takes the agent using the Q-value bounds $\overline{Q}^{\chi}(s', a)$ from before the agent takes \texttt{NOP} and the history of how these bounds have been changing as a result of taking \texttt{NOP} previously. We show one way to produce such estimates in the next subsection.


With post-\texttt{NOP} bounds being sampled from $\overline{\mathcal{Q}}^{\chi'}$, whose distribution approximates BRTDP's configuration-to-configuration transition function $T^{B(M)}(\chi, \chi')$, we can rewrite Equation \ref{eq:qnopapprox} as

\begin{align}\label{eq:qnopapproxrand}
Q^*(s^m, \texttt{NOP}) &\approx \sum_{s'} T(s, \texttt{NOP}, s') E_{\overline{\mathcal{Q}}^{\chi'}} [V^{\chi'}(s')]
\end{align}

To derive the expectation $E_{\overline{Q}^{\chi'}} [V^{\chi'}(s')]$, for any state $s$ we define a random variable $A^*_s$ whose value is action $a$ iff $a$ has the highest Q-value in $s$. Using this variable, Equation \ref{eq:approxQafut} and the fact that, by Equation \ref{eq:maxact}, $V^{\chi'}(s')$ is determined by the highest Q-value of an action in $s'$, we get


%\begin{align}\label{eq:expv}
%E_{\overline{\mathcal{Q}}^{\chi'},\underline{\mathcal{Q}}^{\chi'}} [V^{\chi'}(s')] \approx \sum_a E_{\overline{\mathcal{Q}}^{\chi'},\underline{\mathcal{Q}}^{\chi'}} &[\mathcal{Q}^{\chi'}(s', a) | A^*_{s'} = a]\nonumber \\
%&\cdot P_{\overline{\mathcal{Q}}^{\chi'},\underline{\mathcal{Q}}^{\chi'}}(A^*_{s'} = a)
%\end{align}


\begin{align}\label{eq:expv}
E_{\overline{\mathcal{Q}}^{\chi'},\underline{\mathcal{Q}}^{\chi'}} [V^{\chi'}(s')] \approx \sum_a E[Q^{\chi'}(s', a) | A^*_{s'} = a] P(A^*_{s'} = a),
\end{align}

\noindent
where both $E[Q^{\chi'}(s', a) | A^*_{s'} = a]$ and $P(A^*_{s'} = a)$ implicitly depend on distributions $\overline{\mathcal{Q}}^{\chi'}$ and $\underline{\mathcal{Q}}^{\chi'}$. In particular, as we described, $Q^{\chi'}(s', a)$ is the expectation of $\mathcal{Q}^{\chi'}(s', a)$, a random variable over the interval whose points are distributed according to $\overline{\mathcal{Q}}^{\chi'}$ and $\underline{\mathcal{Q}}^{\chi'}$; in turn, the probability $P(A^*_{s'} = a)$ that $a$'s Q-value is dominant in $s'$ depends on $Q^{\chi'}(s', a')$ for all actions $a'$. 

Based on these observations, simple manipulations yield %Plugging Equation \ref{eq:expv}}


\begin{align}\label{eq:p}
P(A^*_{s'}& = a) =\int\int P(Q^{\chi'}(s', a)) \cdot \\ 
&\cdot \prod_{a' \neq a} P(Q^{\chi'}(s', a) > Q^{\chi'}(s', a')) dQ^{\chi'}(s', a) dQ^{\chi'}(s', a')\nonumber 
%E_{\overline{\mathcal{Q}}^{\chi'},\underline{\mathcal{Q}}^{\chi'}} [V^{\chi'}(s')] \approx \sum_a E[\mathcal{Q}^{\chi'}(s', a) | A^*_{s'} = a] P(A^*_{s'} = a),
\end{align}

\noindent
and

\begin{align}\label{eq:e}
&E[Q^{\chi'}(s', a) | A^*_{s'} = a] = \\
&\int Q^{\chi'}(s', a) \frac{P(A^*_{s'} = a | Q^{\chi'}(s', a)) P(Q^{\chi'}(s', a))}{P(A^*_{s'} = a)} dQ^{\chi'}(s', a) \nonumber
\end{align}


As previously, the probabilities in Equations \ref{eq:p} and \ref{eq:e} are ultimately induced by distributions $\overline{\mathcal{Q}}^{\chi'}$ and $\underline{\mathcal{Q}}^{\chi'}$. In the next subsection we show how appropriate choices of these distributions make Equations \ref{eq:p} and \ref{eq:e} quick to evaluate while yielding good approximation quality. For now, we recap by pointing out that Equation \ref{eq:qnopapproxrand}, whose parts are computed via Equations \ref{eq:expv}, \ref{eq:p}, and \ref{eq:e}, provides us with the desired estimate of $Q^*(s^m, \texttt{NOP})$, and the computation of this estimate is largely enabled by the properties of the BRTDP algorithm.
}

\noindent
\textbf{Estimating $\mathbf{Q^*(s^m, f(s,\chi))}$}. If $a = f(s,\chi)) \neq \texttt{NOP}$, the agent will not do any thinking in the current step.  By meta-myopicity, the agent will not do any thinking after acting either, so we approximate the Q-value of $a$ in the meta-MDP as $Q^*(s^m, f(s,\chi)) = Q^\chi(s, a)$ where $Q^\chi$ is the Q-value function of the policy corresponding to BRTDP's configuration $\chi$. BRTDP's bounds on the MDP's value function immediately give us bounds on $Q^*(s, a)$ in any state $s$. By BRTDP's properties, we know that $Q^*(s, a) \in [\underline{Q}(s,a), \overline{Q}(s, a)]$. While this interval can be large, especially when BRTDP has just started running, we can maintain a \emph{belief distribution} over it, denoted as $\mathcal{Q}(s, a)$. This, in turn, lets us approximate $Q^*(s, a)$, and hence $Q^*(s^m, f(s,\chi))$, with the expectation of the current such belief:

\begin{align}\label{eq:approxQa}
Q^*(s^m, f(s,\chi)) \approx E[\mathcal{Q}(s, a)]
\end{align}
\\

%they allow us to derive one of the quantities we seek, $V^{\chi'}(s')$:

%\begin{align}
%V^{\chi'}(s') = \max_a.
%\end{align}



% that, if we interpret one thinking cycle (i.e., one \texttt{NOP}) execution as running some number of complete BRTDP trials, then \emph{BRTDP's configuration after every cycle is fully determined by the agent's world %state $s$ and BRTDP's current upper and lower bounds on value function}. Let $\overline{V}^{\chi'}(s')$ denote the value of BRTDP's upper bound corresponding to configuration $\chi'$ at world state $s'$.

%Since policies greedy w.r.t. BRTDP's upper bound have the upper bound as their performance guarantee.

\comment{
Intuitively, in order for an agent to solve a metareasoning problem, it must, at every state it encounters, determine whether performing another step of computation will result in greater expected utility than executing its currently suggested action. If it computes that the gain in expected utility from computation, or the \emph{value of computation} (VOC) \cite{russell-aij91,horvitz-ijcai89,horvitz-uai87}  is positive, then it should plan. In this section, we lay the theoretical groundwork for our algorithms by defining the expected VOC in the framework of planning under uncertainty. 

Given an MDP M, its planner B, the resulting metareasoning problem $\texttt{Meta}_{B}(M)$, and the state $s^m = (s, \chi) \in S^m$, the VOC is simply the difference in expected utility of planning for another cycle and acting according to the policy implied by B's current configuration, $\sigma$. Formally,
\begin{align*}
VOC(s^m) =& Q(s^m, f(s,\chi)) - Q(s^m, \texttt{NOP}).  \\
\end{align*}
where $Q$ is the Q-value function of the optimal metareasoning policy. %If the expected value of computation is positive, then the agent should plan for another cycle. Otherwise, the agent should execute its current policy. 
}

\comment{
We now present a series of experiments to show the intelligent behavior of our metareasoning algorithms. Towards this goal, we introduce the concept of the \emph{metareasoning gap}, which we use to characterize the amenability of a domain to metareasoning. The metareasoning gap is simply the ratio of the expected cost of the optimal metareasoning policy to the initial heuristic policy for the base MDP, computed at the initial state. We develop this characterization because constructing an optimal metareasoner is impossible, and approximate metareasoning may not always help the agent with respect to the agent's intiial policy. For example, if the agent's initial policy is the optimal policy, then optimal metareasoning will direct the agent to never think, whereas the chance that any approximate metareasoner makes such a choice is highly unlikely.  


We show in this section that for many domains in which a large metareasoning gap exists (\emph{i.e.,} the ratio is small, and much potential for improvement by metareasoning exists), our algorithms are able to make that improvement, despite our many approximations.

\subsection{Experimental Setup}
In our experiments, we compare our metareasoners against a number of baselines, the first of which is the \texttt{Think$^*$Act} baseline. \texttt{Think$^*$Act} simply plans for $n$ cycles at the initial state and then executes the resulting policy, without ever planning again. We also compare our algorithms to a \texttt{Prob} baseline, which at each state, chooses to plan with probability $p$, and executes its current policy with probability $1-p$.  Note that these baselines are unfair, because the agent does not know a-priori how to set $n$ or $p$. However, they provide useful insight into the optimal metaplanning for various domains. A fairer baseline we compare to is the \texttt{NoInfoThink} agent that simply plans for another cycle if it does not have information about how the upper bounds will change. Our algorithm can then be viewed as an intelligent extension of this baseline that uses information about how the bounds change in order to compute the value of planning. We also show the performance of the initial \texttt{Heuristic}.

We showcase the intelligence of our agent in a wide variety of representative domains that embody the scenarios an agent is likely to encounter in the real-world. In some cases, we will see lackluster performance from our algorithms, and we expect such behavior in domains in which the metareasoning gap is small. All our domains are constructed on top of a vanilla $100\times 100$ GridWorld. Because of space constraints, we only describe the domains at a high level, but full details can be found in the supplemental materials. The initial heuristic for each domain is the Manhattan distance heuristic.

In all our experiments we run each metareasoning algorithm until it reaches the goal. We repeat each experiment 1000 times and present the average cost to the goal to account for stochasticity in the domain, algorithms, and BRTDP. Finally, each BRTDP trajectory is 50 actions long.

\subsection{Results}
We do not present experiments in the vanilla domain, because the heuristic induces the optimal policy, resulting in a metareasoning gap of 0. Our agent would perform quite poorly, since spending any amount of time thinking is suboptimal. Therefore, we begin with a domain in which we add "winds" that can push the agent around, in order to prevent a basic heuristic from being the optimal policy. In fact, in this domain, an optimal agent must move against its heuristic to reach an area where the winds can quickly push it to the goal. In these experiments, we vary the cost of \texttt{NOP} as well as the cost of taking a base-level action.  

Because of lack of space, we move most of the graphs showing the results to the supplementary materials, and just describe the general trends. We see that as we increase the cost of thinking, policies that value less thinking start to do better. For instance, when the cost of thinking is low, \texttt{Think*Act} does well when $n$ is high and \texttt{Prob} does well when $p$ is high, and when the cost of thinking is high, \texttt{Think*Act} does well when $n$ is low and \texttt{Prob} does well when $p$ is low. Because increasing the cost of acting is similar to decreasing the cost of thinking We see similar results when we vary the cost of acting. The metareasoning gaps in this domain are extremely large, and in all settings we see that \texttt{Metareasoner} performs the best and is able to close this metareasoning gap significantly. Figure \ref{winds-dCOT-average} shows our results averaged over all cost of thinking settings.
We leave out \texttt{Heuristic} (whose cost is 1089) to make the graph more readable. Importantly, we see that \texttt{Metareasoner} performs better than \texttt{NoInfoThink}, which shows that it is making intelligent decisions after it learns about how the bounds on q-values will change.  \texttt{UnCorr Metareasoner} does not do as well as \texttt{Metareasoner}, probably because the assumption that the actions are not correlated is not a good one.

\begin{figure}
\centering
\includegraphics[scale = 0.45]{figures-winds-dCOT-average.pdf}
\caption{When averaged over all settings of the cost of thinking, \texttt{Metareasoner} results in a lower average cost to the goal than all parameter settings for all baselines.}
\label{winds-dCOT-average}
\end{figure}

We now turn to a domain in which costs are not uniform. We make acting and thinking far more costly in the initial state than in others. Figure \ref{lavapit} shows the result. As expected, \texttt{Heuristic} does extremely poorly. \texttt{Think*Act} and \texttt{Prob} both perform poorly when they encourage lots of thinking. \texttt{Think*Act} performs particularly poorly as $n$ increases, because it spends all its time in the initial state. \texttt{Metareasoner} is again able to close the large metareasoning gap that exists, and performs the best, because it is able to figure out that it should not think in its initial state (beyond the initial thinking step), and instead should quickly leave the initial state and then do its planning in other, safer, states. \texttt{Uncorr Metareasoner} also closes the metareasoning gap significantly, but again does not perform as well as \texttt{Metareasoner}.


\begin{figure}
\centering
\includegraphics[scale = 0.45]{figures-lavapit-strongerbaseline-1.pdf}
\caption{A domain in which acting and thinking is far more costly in the initial state than in other states.}
\label{lavapit}
\end{figure}

In the previous experiments, we have looked at domains in which the cost of thinking is explicit. We now investigate domains with nonstationary \texttt{NOP}s, in which the cost of thinking is implicit, in that executing a \texttt{NOP} can move the agent away from the goal.  Taking a \texttt{NOP} adds costs that are not myopically obvious. We also take this concept to the extreme by modifying the wind patterns so that most of them move the agent away from the goal. Figure \ref{fireants1} shows the results. We see that the \texttt{Prob} baseline perform particularly poorly and that both \texttt{Heuristic} and many settings of \texttt{Think*Act} do better. We also see that our algorithms do not show the large gains we saw in earlier domains. However, this result is not surprising, because this domain is designed precisely to defeat our algorithms. Each time the agent chooses to think, it gets pushed away from the goal. Moreover, not only does it get pushed away from the goal, it likely gets pushed into a state it has never encountered before, and then it must think again because of lack of information. If the agent is unable to quickly discover the very few jetstreams that can quickly push it towards the goal, it will be trapped. As we would expect, the metareasoning gap of this domain is quite small in comparison to the previous domains, because the initial heuristic doesn't fall into such traps. 

We next modify this domain by increasing the availability of winds that can push the agent toward its goal, so that the agent is not forever doomed. The new winds provide the agent an opportunity to recover, and instead of directly increasing the metareasoning gap of the initial state, increases the metareasoning gap in many other states. We see in Figure \ref{fireants2} that both \texttt{Metareasoner} and \texttt{UnCorr Metareasoner} now do a much better job of closing the metareasoning gap.



\begin{figure}
\centering
\includegraphics[scale = 0.45]{figures-windsthatmove-noNjet-strongerbaseline-1.pdf}
\caption{When \texttt{NOP}s are nonstationary, our algorithms are still powerful, but do not show the huge gains as in earlier domains.}
\label{fireants1}
\end{figure}
\begin{figure}
\centering
\includegraphics[scale = 0.45]{figures-windsthatmove-strongerbaseline-2-1.pdf}
\caption{When we increase the likelihood of recovery, our algorithm again perform well compared to the baselines.}
\label{fireants2}
\end{figure}
}



\comment{
\subsection{Metareasoning Gap}
We now quantify the metareasoning gap in our domains. However,
computing the metareasoning gap exactly is difficult, because it requires computation of the optimal metareasoning policy. Instead, we compute an upper bound on the metareasoning gap by substituting the cost of the optimal metareasoning policy with the cost of the optimal policy for the base MDP. The metareasoning gap can be no larger than this upper bound, because metareasoning only adds cost to the optimal base policy. We show the metareasoning gaps for each domain that we consider in Table \ref{MG}.

Table \ref{MG} shows that Domain Type 5 actually has a narrower metareasoning gap than Domain Type 4, but in this case, we must consider the metareasoning gap in states other than the initial state. 
By adding the Easterly Winds, the metareasoning gap in states that used to be trap states is significantly widened, giving metareasoners the opportunity to make gains in those states. 
%\begin{table}[h]
%\begin{tabular}{@{}llllll@{}}
%\toprule
%         & Heuristic & UCT & Optimal Policy & MG$^{UB}$ &  \\ \midrule
%Lavapit &   979 &   222.78 & 113.516   & 0.116   &  \\
%JetStream &  119.364 &  118.203  &   66 &  0.331 &\\
%No JetStream &  251.438  & 499.226   &  66  & 0.262 & \\
%COA = 1  & 99  &  & 8.873                  &  0.09 &\\
%COA = 5  & 495 &  & 43.992                  &  0.09 &\\
%COA = 10 & 990 &  & 87.898                  &  0.09 &\\
%COA = 15 & 1485  &  & 131.824                  &  0.09 &\\
%COT = 1& 1089  & & 103.9                  &  0.095 &\\
%COT = 5 & 1089 &  & 103.9                  & 0.095 \\
%COT = 10& 1089 &  & 103.9                  & 0.095 \\
%COT = 15 & 1089 &  & 103.9                  & 0.095 \\
%Avg COA &  &  &                   &  \\
%Avg COT &  &  &                   &  \\ \bottomrule
%\end{tabular}
%\end{table}
\begin{table}
\begin{tabular}{@{}lllll@{}}
\toprule
         & Heuristic & Optimal Base Policy & MG$^{UB}$ &  \\ \midrule
Lavapit &   979 &  113.516   & 0.116   &  \\
JetStream &  119.364 &   66 &  0.331 &\\
No JetStream &  251.438  &  66  & 0.262 & \\
COA = 1  & 99   & 8.873                  &  0.09 &\\
COA = 5  & 495   & 43.992                  &  0.09 &\\
COA = 10 & 990   & 87.898                  &  0.09 &\\
COA = 15 & 1485    & 131.824                  &  0.09 &\\
COT = 1& 1089   & 103.9                  &  0.095 &\\
COT = 5 & 1089   & 103.9                  & 0.095 \\
COT = 10& 1089   & 103.9                  & 0.095 \\
COT = 15 & 1089   & 103.9                  & 0.095 \\
%Avg COA &  &  &                   &  \\
%Avg COT &  &  &                   &  \\ 
\bottomrule
\end{tabular}
\caption{The average cost of the heuristic, the average cost of the optimal base policy, and upper bounds on the metareasoning gaps for each domain.}
\label{MG}
\end{table}
%\begin{figure}
%\centering
%\begin{subfigure}[b]{0.2\textwidth}
%\includegraphics[width=\textwidth]{gap1.PNG}
%\caption{Easterly Jet Stream}
%\label{Njet}
%\end{subfigure}
%\qquad
%\begin{subfigure}[b]{0.2\textwidth}
%\includegraphics[width=\textwidth]{gap2.PNG}
%\caption{No Eastery Jetstream}
%\label{noNjet}
%\end{subfigure}
%\caption{Metareasoning gaps for two domains.}
%\label{gap}
%\end{figure}
}
